$k$-local Graphs

In 2017 Day et al. introduced the notion of locality as a structural complexity-measure for patterns in the field of pattern matching established by Angluin in 1980. In 2019 Casel et al. showed that determining the locality of an arbitrary pattern is NP-complete. Inspired by hierarchical clustering, we extend the notion to coloured graphs, i.e., given a coloured graph determine an enumeration of the colours such that colouring the graph stepwise according to the enumeration leads to as few clusters as possible. Next to first theoretical results on graph classes, we propose a priority search algorithm to compute the $k$-locality of a graph. The algorithm is optimal in the number of marking prefix expansions, and is faster by orders of magnitude than an exhaustive search. Finally, we perform a case study on a DBLP subgraph to demonstrate the potential of $k$-locality for knowledge discovery.

==> proofs/non-connected.tex <==

	In our work we decided to only investigate connected graphs after we connected the locality to the number of connected components.
	Here we present that the problem does not become any easier by this restriction.
	
	\begin{problem}
		For an undirected connected graph $G=(V,E)$, a colouring~$c\colon
		V\to\{1,\dots,|V|\}$ and a number $k\in\mathbb{N}$, we define the problem $\ConLoc$ by $(G,c,k) \in \ConLoc$ iff there exists ordering $(c_1,\dots, c_t)$ of all the colours in
		$\mathcal{C}(G,c)$ such that for every $i\in\{1,\dots, t\}$ we have at most $k$ connected components in $G|_{\bigcup_{j = 1}^i c_j}$.
	\end{problem}
	
	\begin{corollary}
		$\ConLoc\leq_{\mathit{fpt}} \Loc_G$.
	\end{corollary}
	
	Unfortunately the same holds for the reverse direction:
	\begin{theorem}
		$\Loc_G\leq \ConLoc$.
	\end{theorem}
	\begin{proof}
		Let $(G,c,k)$ be an instance for $\Loc_G$. If $G$
		has only one connected component we are done. Otherwise, add $k+1$
		vertices $V_x$ for every colour~$x$ that occurs in $G$. Then connect all
		vertices of $G$ coloured in $x$ with all vertices $V_x$. Pick one new
		colour $x^*$ and assign it to all new vertices. 
		
		Observe that any ordering that certifies that $(G,c)$ is $k$-local
		can be extended by adding $x^*$ at the end to certify that the
		resulting graph is $k$-local. For the other direction, note that in
		any valid colour ordering the new colour must occur after any other
		colour that occurred in the initial graph. Otherwise if we pick all
		colours except the last one $x'$, then $V_x'$ will be part of the
		induced graph $G|_{\bigcup_{i=1}^{|V|} c_i}$. And then, we have at
		least $k+1$ connected components. Therefore, we can assume that any
		valid ordering for the resulting graph that satisfies its
		$k$-locality ends with the new colour. Therefore, by removing  the
		last colour we only have the initial colours and therefore induce the
		whole graph $G$.
	\end{proof}


==> proofs/priority_search_full.tex <==

\begin{proof}
    According to Lemma \ref{priority_search_lemma1} we must continue to expand marking prefixes, as long as incomplete marking prefixes remain at the front of the queue with $k$-locality less than $\kappa$.
    According to Lemma \ref{priority_search_lemma2} the relevant marking prefixes reside at the front of the queue and are expanded from there.
    According to Lemma \ref{priority_search_lemma3}, the marking prefixes are expanded as long as they have a $k$-locality less than or equal to $\kappa$.
    In total, this proves that Algorithm \ref{alg:priority_search} guarantees correct results, since it expands at least all necessary marking prefixes, and is optimal, because it never expands any unnecessary marking prefixes.
\end{proof}



==> proofs/priority_search_pt1.tex <==

\begin{proof}
    Assume that a marking prefix $p$ with $\loc(G,p) \leq \kappa$ is not expanded by a correct algorithm.
    Then it is still possible for an expansion $p'$ of $p$ to have $\loc(G, p') \leq \kappa$.
    The minimum $k$-locality of $G$ w.r.t. all marking sequences could not be validated, and $p'$ (or an expansion thereof) could be part of the result (i.e., $M$).
    This would violate the assumption of correctness.
\end{proof}

==> proofs/priority_search_pt2.tex <==

\begin{proof}
    All marking prefixes are expanded in the order they are taken from the queue.
    Since the queue is always maintained sorted in ascending order w.r.t.~the $k$-locality, they are taken from the queue in ascending order.
    As a result, we must ensure that no marking prefix $p'$ with lower $k$-locality than a previously accessed marking prefix $p$ is added into the queue (where it later could be accessed and expanded again, violating the expansion in ascending order).
    If a marking prefix $p''$ was taken from the queue after $p$, it was either sorted behind $p$ because it had a greater or equal $k$-locality to begin with, or it is an expansion of $p$, in which case it cannot have lower $k$-locality, since current$_k$ in line 9 can never shrink.
    Therefore, all marking prefixes that are added to the queue later must have a greater or equal $k$-locality, ensuring that the marking prefixes are accessed and expanded in ascending order w.r.t.~the $k$-locality.
\end{proof}


==> proofs/priority_search_pt3.tex <==

\begin{proof}
    The variable min$_k$ is only set once a marking prefix is expanded to a complete marking sequence $e$.
    If $\loc(G, e) = \kappa$, the condition in line 4 guarantees that no further marking prefixes with larger $k$-locality are expanded.
    If $\loc(G,e) > \kappa$, then, according to Lemma \ref{priority_search_lemma2}, the $k$-locality of its un-expanded version must have had a lower $k$-locality than any marking prefix in $M'$, since it was expanded first.
    As such, the prefix of $e$ must have had a $k$-locality of at most $\kappa$.
\end{proof}


==> rammodel.tex <==
The computational model we use is the standard unit-cost RAM with logarithmic word size: for an input of size $n$, each memory word can hold $\log (n)$ bits. Arithmetic and bitwise operations with numbers in $[1,n]$ are, thus, assumed to take $O(1)$ time. Numbers larger than $n$, with $\ell$ bits, are represented in $O(\ell/\log n)$ memory words, and working with them takes time proportional to the number of memory words on which they are represented. In all the problems, we assume that we are given a number $k$, binary encoded, and a finite, undirected graph $G$, specified as the set of vertices and the set of edges. The size of the input is, as such, the size of the binary encoding of $k$, which is $\lceil\log_2 k\rceil$, plus the size $S$ of the graph $G$. So, one memory word can hold $\log (S+\log_2 (k))$ bits.

For a more detailed general discussion on this model see, e.\,g.,~\cite{crochemore}. 

%Some of our algorithms run in exponential time and use exponential space w.r.t. the size $n$ of the input. Following the literature dealing with such exponential algorithms (see, e.g., \cite{FominKTV08}), we will use the $O^*$-notation. By definition, for functions $f$ and $g$ we write $f(n) = O^*(g(n))$ if $ f(n)=O(g(n)n^{O(1)})$. In other words, the $O^*$-notation hides polynomial factors, just as the $O$-notation hides constants. Using this notation, we can assume that our single-exponential time and single-exponential space algorithms run on a RAM model where arithmetic and bitwise operations with single exponential numbers (w.r.t. the size $n$ of the input) as well as accessing the memory-words (given their address, like in an usual RAM) are assumed to take $O^*(1)$ time. Working with such a computational model allows us to analyse the actual algorithms rather than the various intricacies of the computational model.
%
%In particular, when expressing the complexity of our algorithms, we get functions which are exponential in $\sigma$ (the size of the alphabet) but polynomial in the number $n$ of states of the input NFA or, for the enumeration algorithms, in the length $m$ of the enumerated strings or in the value of the input number $k$ (the parameter of the considered problems). For clarity of the exposure, although we use the $O^*$-notation, we will explicitly write the dependency on $n, m,$ and $k$, and only hide the polynomial dependency on $\sigma$. 

==> shortcuts.tex <==
\ProvidesPackage{shortcuts}

\RequirePackage{amsmath}
\RequirePackage{mathtools}

\def\ta{\mathtt{a}}
\def\tb{\mathtt{b}}
\def\tc{\mathtt{c}}
\def\td{\mathtt{d}}
\def\te{\mathtt{e}}
\def\tm{\mathtt{m}}
\def\tn{\mathtt{n}}
\def\tp{\mathtt{p}}
\def\tx{\mathtt{x}}
\def\ty{\mathtt{y}}
\def\tz{\mathtt{z}}

\def\toa{\overline{\mathtt{a}}}
\def\top{\overline{\mathtt{p}}}
\def\toy{\overline{\mathtt{y}}}



\def\tzero{\mathtt{0}}
\def\tone{\mathtt{1}}
\def\ttwo{\mathtt{2}}
\def\r{\operatorname{r}}
\def\re{\operatorname{r}}
\def\m{\operatorname{m}}

\def\etal{\emph{et al. }}


\def\nth#1{#1$^{\text{th}}$}
\def\nst#1{#1$^{\text{st}}$}
\def\nnd#1{#1$^{\text{nd}}$}
\def\nrd#1{#1$^{\text{rd}}$}


\def\abs#1{|#1|}


% Redefine epsilon
\renewcommand{\epsilon}{\varepsilon}
% Redefine phi
\renewcommand{\phi}{\varphi}


\def\N{\mathbb{N}} %natural numbers
\def\Z{\mathbb{Z}} %natural numbers
\def\P{\mathbb{P}} %prime numbers


\DeclareMathOperator\ScatFact{SubSeq}
\DeclareMathOperator\AbsScatFact{AbsSubSeq}
\DeclareMathOperator\SubWords{SubSeq}
\DeclareMathOperator\SubSeq{SubSeq}
\DeclareMathOperator{\al}{alph}
\DeclareMathOperator{\alphabet}{alph}
\DeclareMathOperator{\letters}{alph}
\DeclareMathOperator{\Fact}{Fact}
\DeclareMathOperator{\Pref}{Pref}
\DeclareMathOperator{\Suff}{Suff}
\DeclareMathOperator{\PerfUniv}{PUniv}
\DeclareMathOperator{\NUniv}{NUniv}
\DeclareMathOperator{\Univ}{Univ}
\DeclareMathOperator{\inner}{in}
\DeclareMathOperator{\archFac}{archFac}
\DeclareMathOperator{\PP}{PP}
\DeclareMathOperator{\NEG}{NEG}
\DeclareMathOperator{\LCR}{LCR}
\DeclareMathOperator{\merge}{merge}

\DeclareMathOperator{\cond}{cond}
\DeclareMathOperator{\ar}{ar}
\DeclareMathOperator{\pdot}{\overline{\cdot}}
\DeclareMathOperator{\colour}{colour}
\def\NP{\textsf{NP}}
\def\Loc{\textsf{Loc}}
\def\ConLoc{\textsf{ConLoc}}
\DeclareMathOperator{\Pos}{Pos}
\DeclareMathOperator{\loc}{loc}
\DeclareMathOperator{\parity}{parity}
\DeclareMathOperator{\odd}{odd}
\DeclareMathOperator{\even}{even}

\newcommand*\colvec[1]{\bigl(\begin{smallmatrix}#1\end{smallmatrix}\bigr)}

\usepackage{bbm}
\def\neutr{\mathbbm{1}} %neutral element

\DeclareMathOperator{\maxpos}{maxpos}
\DeclareMathOperator{\minpos}{minpos}
\DeclareMathOperator{\pos}{pos}

\DeclareMathOperator{\dom}{dom}
\DeclareMathOperator{\lex}{lex}

\DeclarePairedDelimiter\card{\lvert}{\rvert}
\DeclarePairedDelimiter\paren{(}{)}
\DeclarePairedDelimiter\set{\{}{\}}

\newcommand{\rev}[1]{\mathpalette\harpoonvec{#1}}
\newcommand{\harpvecsign}{\scriptscriptstyle\leftharpoonup}
\newcommand{\harpoonvec}[2]{%
  \ifx\displaystyle#1\doalign{$\harpvecsign$}{#1#2}\fi
  \ifx\textstyle#1\doalign{$\harpvecsign$}{#1#2}\fi
  \ifx\scriptstyle#1\doalign{\scalebox{.6}[.9]{$\harpvecsign$}}{#1#2}\fi
  \ifx\scriptscriptstyle#1\doalign{\scalebox{.5}[.8]{$\harpvecsign$}}{#1#2}\fi
}
\newcommand{\doalign}[2]{%
 {\vbox{\offinterlineskip\ialign{\hfil##\hfil\cr#1\cr$#2$\cr}}}%
}
\DeclareMathOperator\w{\rev\m}
\DeclareMathOperator\ra{\rev\ar}
\DeclareMathOperator\er{\rev\r}

\DeclareMathOperator{\AS}{AS}

\DeclareMathOperator{\posToArch}{posToArch}
\DeclareMathOperator{\firstInArch}{firstInArch}
\DeclareMathOperator{\ExtSet}{ExtSet}
\DeclareMathOperator{\ExtPos}{ExtPos}
\DeclareMathOperator{\EnumSF}{EnumSF}

\usepackage{cleveref}

